A thermo-diffusion system with Smoluchowski interactions: well-posedness and homogenization

We study the solvability and homogenization of a thermal-diffusion reaction problem posed in a periodically perforated domain. The system describes the motion of populations of hot colloidal particles interacting together via Smoluchowski production terms. The upscaled system, obtained via two-scale convergence techniques, allows the investigation of deposition effects in porous materials in the presence of thermal gradients.

==> minilib.tex <==
\usepackage{xstring}
\usepackage{xargs}
\usepackage{etoolbox}
\makeatletter
% ===constructor=======================================================================================
% 1:   command name
% 2:   glyph
% the new command will function similarly to a dict with error checking
\newcommand\constructor[2]{
  \expandafter\newcommandx\csname #1\endcsname[2][1=,2=]{\ifstrequal{##1}{}
    {#2}
    {\@ifundefined{#1@##1}
      {\errmessage{"#1" has no field named "##1"}}
      {\ifstrequal{##2}{}
        {\@nameuse{#1@##1}}
        {\@ifundefined{\@nameuse{#1@##1}@##2}
          {\errmessage{"\@nameuse{#1@##1}" has no field named "##2"}}
          {\@nameuse{\@nameuse{#1@##1}@##2}}}
      }
    }
  }
  \@namedef{#1@self}{#2}
}
% ———setter————————————————————————————————————————————————————————————————————————
\newcommand\set[3]{             % this, field, value
  \@namedef{#1@#2}{#3}
}
% ———getter————————————————————————————————————————————————————————————————————————
\def\ifstrequalx#1{\edef\@t{#1}\expandafter\ifstrequal\expandafter{\@t}}
\newcommand\cget[2]{\@ifundefined{#1@#2}{\errmessage{"#1" has no field named "#2"}}{\@nameuse{#1@#2}}}
% this one can't be used as argument of other command for some reason
\newcommandx\get[5][3=,4=,5=]{\ifstrequal{#3}{}
  {\cget{#1}{#2}}{\ifstrequal{#4}{}
    {\cget{\cget{#1}{#2}}{#3}}{\ifstrequal{#5}{}
      {\cget{\cget{\cget{#1}{#2}}{#3}}{#4}}
      {\cget{\cget{\cget{\cget{#1}{#2}}{#3}}{#4}}{5}}}}}
\newcommand\self[1]{\@nameuse{#1@self}}
% ===defineDomain======================================================================================
% 1:   command name
% 2:   variable glyph
% 3:   glyph
% 4:   "in" or "on", default is in.
% e.g. \defineDomain{G}{x}{\Gamma}[on]
\newcommandx\defineDomain[4][4=in]{
  \constructor{#1}{#3}                                % e.g. \G:=\Gamma
  \set{#1}{dim}{1}                                    % e.g. \G[dim]:=1
  \set{#1}{domain}{#1}                                % e.g. \G[domain]:=G
  \set{#1}{var}{#2}                                   % e.g. \G[var]:=x
  \set{#1}{on}{#4}                                    % e.g. \G[on]:=on
}
% ———operations————————————————————————————————————————————————————————————————————
% \attachIntegral{G}{\int\int_{\G}}                   % e.g. \int[G]:=\int\int_{\G}
\newcommand\renewInt[2]{
  \set{#1}{int}{#2}
}
% redefine \int to accept one optional argument
\let\oldInt\int
\renewcommandx\int[1][1=]{\ifstrequal{#1}{}
  {\oldInt}
  {\intx{#1}}
}
\newcommand\intx[1]{
  \@ifundefined{#1@int}
  {\int\limits_{\self{#1}}}
  {\@nameuse{#1@int}}
}
% ===defineCrossProduct================================================================================
% 1:   command name
% 2:   domain 1
% 3:   domain 2
% e.g. \defineCrossProduct{TG}{Time}{G}
\newcommand\defineCrossProduct[3]{
  \constructor{#1}{\self{#2}\times\self{#3}}          % \TG:=(0,T)\times\Gamma
  \set{#1}{dim}{2}                                    % \TG[dim]:=2
  \set{#1}{var}{(\get{#2}{var},\get{#3}{var})}        % \TG[var]:=(t,x)
  \set{#1}{d1}{#2}                                    % \TG[1][var]:=(0,T)
  \set{#1}{d2}{#3}                                    % \TG[2][var]:=\Gamma
  \@attachInOn{#1}{#2}{#3}                            % \TG[on]:=on
  \set{#1}{domain}{#1}                                % \TG[domain]:=TG
  \set{#1}{int}{\intx{#2}\intx{#3}}                   % \intx{TG}:=\int_0^T\int_\Gamma
}
% ———getBoundary———————————————————————————————————————————————————————————————————
\newcommand\getBoundaryEx[2]{\@ifundefined{#1@#2}
  {\get{#1}{self}}
  {\get{#1}{#2}}
}
\newcommand\getBoundary[2]{\ifstrequalx{\cget{#1}{dim}}{1} % 1 or 2
  {\cget{#1}{#2}}
  {\getBoundaryEx{\cget{#1}{d1}}{#2}\times\getBoundaryEx{\cget{#1}{d2}}{#2}}
}
% ———ifstrequalx———————————————————————————————————————————————————————————————————
% it's ~ \ifstrequal, except it evaluates its first argument
\def\ifstrequalx#1{\edef\@t{#1}\expandafter\ifstrequal\expandafter{\@t}}
\newcommand\@attachInOn[3]{
  % inherit "on" text with || of #2 and #3
  \@namedef{#1@on}{in}
  \ifstrequalx{\@nameuse{#3@on}}{on}{\@namedef{#1@on}{on}}{}
  \ifstrequalx{\@nameuse{#2@on}}{on}{\@namedef{#1@on}{on}}{}
}
% ===defineBoundarySegment=============================================================================
% e.g. \defineBoundarySegment{G}{A}{Grain}{\Gamma}
\newcommand\defineBoundarySegment[4]{ % boundary, segment type, glyph
  \defineDomain{#1}{\get{#2}{var}}{#4}[on]
  \set{#2}{#3}{#4}
  \set{#2}{ref#3}{#1}
}
\newcommandx\getdomain[2][2=]{\ifstrequal{#2}{}
  {\@nameuse{#1@domain}}
  {\@nameuse{\@nameuse{#1@domain}@d#2}}
}
% ===defineUnknown=====================================================================================
% 1: command name
% 2: glyph
% 3: domain of definition
% e.g. \defineUnknown{temp}{\theta}{TA}
\newcommand\defineUnknown[3]{
  \constructor{#1}{#2}
  \set{#1}{parent}{}
  \set{#1}{domain}{#3}
}
% ———operations————————————————————————————————————————————————————————————————————
% e.g. \attachFlux{coll}{\diff}
\newcommand\attachFlux[2]{
  \set{#1}{coeff}{#2}
}
\newcommand\flux[1]{
  \get{#1}{coeff}\nabla \self{#1}
}
% ===inheritUnknown====================================================================================
% 1: parent
% 2: command name
% 3: glyph
% e.g. \inheritUnknown{coll}{coll_i}{u_i}
\newcommand\inheritUnknown[3]{
  \set{#2}{parent}{#1}
  \set{#2}{self}{#3}
  \set{#2}{domain}{\@nameuse{#1@domain}}
  \set{#2}{vector}{\self{#1}}
}
% ———tdomain———————————————————————————————————————————————————————————————————————
\newcommandx\tdomain[2][2=]{\ifstrequal{#2}{}{\indomain{\cget{#1}{domain}}}
  {\ifstrequal{#2}{1}{\indomain{\cget{\cget{#1}{domain}}{d1}}}
    {\ifstrequal{#2}{2}{\indomain{\cget{\cget{#1}{domain}}{d2}}}
      {\text{on }\getBoundary{\cget{#1}{domain}}{#2}}}}}
% ———indomain——————————————————————————————————————————————————————————————————————
\newcommand\indomain[1]{
  \text{\get{#1}{on} }\get{#1}{self}
}
\makeatother
% ===Lebesgue spaces===================================================================================
\newcommand\Li[1]{
  L^\infty(\self{#1})
}
\newcommand\Lp[1]{
  L^p(\self{#1})
}
\newcommand\Lt[1]{
  L^2(\self{#1})
}
\newcommand\forAll[1]{
  \text{for all }\get{#1}{var}\in\get{#1}{self}
}

==> subsup.tex <==
\usepackage{xargs}
\usepackage{etoolbox}
\newcommand\commajoin[2]{{#1,#2}}
\newcommand\plainjoin[2]{{#1#2}}
\makeatletter
% ===newsubsupcommand==================================================================================
% usage:
% \newsubsupcommand
%   {<command name>}
%   {<variable name>}
%   [{<default subscript>}]       -- defualts to empty
%   [{<default superscript>}]     -- defaults to empty
%   [<subscript join function>]   -- defaults to comma
%   [<superscript join function>] -- defaults to comma
%
% When the defined command is used with a subscript or superscript or both,
% they will be joinded by the appropriate join function to the default sub/super-scripts.
%
% Example:
%
% \newsubsupcommand{\yab}{y}[a][b]
%
% $\yab$      := $y_{a}^{b}$
% $\yab_c$    := $y_{a,c}^{b}$
% $\yab^d$    := $y_{a}^{b,d}$
% $\yab_c^d$  := $y_{a,c}^{b,d}$
%
% \newsubsupcommand{\ya}{y}[a]
% \newsubsupcommand{\yb}{y}[][b]

% \newcommandx\sswrap[5]{
%   #1\sub@sup{#2}{#3}{#4}{5}
% }

\newcommand\newifsubcommand[3]{\newcommand#1{\@ifnextchar_{#2}{#3}}}
\newcommandx\newsubsupcommand[6][3=,4=,5=\commajoin,6=\commajoin]{
  \ifstrequal{#4}{}
  {
    \ifstrequal{#3}{}
    {\newcommand#1{#2}}
    % else
    {\newcommand#1{#2\sub@{#3}{#5}}}
  }
  % else
  {
    \ifstrequal{#3}{}
    {\newcommand#1{#2\sup@{#4}{#6}
      }}
    % else
    {\newcommand#1{#2\sub@sup{#3}{#4}{#5}{#6}}}
  }
}
\def\sub@#1#2{
  \def\default@sub{#1}
  \def\sub@merger{#2}
  \@ifnextchar_
  {\merge@sub}
  {_{\default@sub}}
}
\def\sup@#1#2{
  \def\default@sup{#1}
  \def\sup@merger{#2}
  \@ifnextchar_
  {\plain@sup}
  {\@ifnextchar^
    {\merge@sup}
    {^{\default@sup}}
  }
}
\def\plain@sup_#1{_{#1}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}
\def\sub@sup#1#2#3#4{
  \def\default@sub{#1}
  \def\default@sup{#2}
  \def\sub@merger{#3}
  \def\sup@merger{#4}
  \@ifnextchar_
  {\merge@sub@sup}
  {\@ifnextchar^
    {_{\default@sub}\merge@sup}
    {_{\default@sub}^{\default@sup}}
  }
}
\def\merge@sub_#1{_{\sub@merger{\default@sub}{#1}}}
\def\merge@sup^#1{^{\sup@merger{\default@sup}{#1}}}
\def\merge@sub@sup_#1{_{\sub@merger{\default@sub}{#1}}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}

\def\tail@sup#1#2{
  \def\default@sup{#1}
  \def\sup@merger{#2}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}

% \if@sub{<do this if there's a subscript ahead, \@sub is the subscript in this context>}
%        {<do this otherwise>}

\def\if@sub#1#2{
  \@ifnextchar_{
    \def\@statement{#1}
    \@apply@sub}
  {#2}
}
\def\@apply@sub_#1{\def\@sub{#1}\@statement}


\makeatother
\newsubsupcommand{\yab}{y}[a][b]

